Numerical simulation of fundamental trapped sausage modes

Context: We integrate the 2D MHD ideal equations of a straight slab to simulate observational results associated with fundamental sausage trapped modes. Aims: Starting from a non-equilibrium state with a dense chromospheric layer, we analyse the evolution of the internal plasma dynamics of magnetic loops, subject to line-tying boundary conditions, and with the coronal parameters described in Asai et al. (2001) and Melnikov et al. (2002) to investigate the onset and damping of sausage modes. Methods: To integrate the equations we used a high resolution shock-capturing (HRSC) method specially designed to deal appropriately with flow discontinuities. Results: Due to non-linearities and inhomogeneities, pure modes are difficult to sustain and always occur coupled among them so as to satisfy, e.g., the line-tying constraint. We found that, in one case, the resonant coupling of the sausage fundamental mode with a slow one results in a non-dissipative damping of the former. Conclusions: In scenarios of thick and dense loops, where the analytical theory predicts the existence of fundamental trapped sausage modes, the coupling of fast and slow quasi-periodic modes -with a node at the center of the longitudinal speed- occur contributing to the damping of the fast mode. If a discontinuity in the total pressure between the loop and the corona is assumed, a fundamental fast sausage transitory leaky regime is spontaneously produced and an external compressional Alfv\'en wave takes away the magnetic energy.

==> graphicx.tex <==
% Plain TeX interface to graphicx package.
% David Carlisle


\input miniltx

\def\Gin@driver{dvips.def}
\input graphicx.sty


\resetatcatcode



